Constrained Learning for Decentralized Multi-Objective Coverage Control

The multi-objective coverage control problem requires a robot swarm to collaboratively provide sensor coverage to multiple heterogeneous importance density fields IDFs simultaneously. We pose this as an optimization problem with constraints and study two different formulations: (1) Fair coverage, where we minimize the maximum coverage cost for any field, promoting equitable resource distribution among all fields; and (2) Constrained coverage, where each field must be covered below a certain cost threshold, ensuring that critical areas receive adequate coverage according to predefined importance levels. We study the decentralized setting where robots have limited communication and local sensing capabilities, making the system more realistic, scalable, and robust. Given the complexity, we propose a novel decentralized constrained learning approach that combines primal-dual optimization with a Learnable Perception-Action-Communication (LPAC) neural network architecture. We show that the Lagrangian of the dual problem can be reformulated as a linear combination of the IDFs, enabling the LPAC policy to serve as a primal solver. We empirically demonstrate that the proposed method (i) significantly outperforms state-of-the-art decentralized controllers by 30% on average in terms of coverage cost, (ii) transfers well to larger environments with more robots, and (iii) scalable in the number of IDFs and robots in the swarm.

==> experiments1.tex <==
\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{plots/fair_plots_1_25.pdf}
	\caption{Fair multi-objective coverage control problem with $32$ robots and $4$ IDFs in a $1024\times 1024$ \SImsqr{} environment. The coverage cost increase in comparison to the clairvoyant is $81\%$, $246\%$, $250\%$, and $258\%$ for LPAC, Centralized, Decentralized, and SFCC \cite{malenciafair} respectively. 
 }
	\label{fig:fair_coverage}
\end{figure}
\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{plots/comm_radius.pdf}
  \caption{Fair coverage control with the LPAC controller normalized by the CVT controller for various communication radius and sensor sizes.\label{fig:comm_radius}}
\end{figure}
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{plots/env_72_plots_1_25.pdf}
  \caption{Performance and dual variables per IDF as a function of time for $32$ robots and $4$ IDFs. Each color represents a different IDF.}\label{fig:fair_objective_dual_variables}
\end{figure}

\begin{table}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \caption{Fair Coverage: Varying Number of Robots}%
  \label{tab:centralized_vs_lpac_fair_robot_ablation}%
  \begin{tabular}{ccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\# Robots}} &\multicolumn{2}{c}{\# Best Environments} & \multicolumn{2}{c}{Average Max Objective }\\\cmidrule(l){2-3} \cmidrule(l){4-5}
    \multicolumn{1}{c}{} & \multicolumn{1}{r}{Centralized CVT} & \multicolumn{1}{r}{LPAC} & \multicolumn{1}{r}{Centralized  CVT} & \multicolumn{1}{r}{LPAC}\\\midrule
8 & 32 & 68 & 2.839&2.763 \\
16 & 15 & 85 & 2.680&2.191 \\
24 & 4 & 96 & 2.559&1.687 \\
32 & 6 & 94 & 2.251&1.386 \\
40 & 2 & 98 & 2.167&1.191 \\
48 & 6 & 94 & 1.842&1.163 \\
56 & 3 & 97 & 1.744&0.981 \\
64 & 3 & 97 & 1.608&0.983 \\
    \bottomrule
  \end{tabular}
\end{table}
\begin{table}
  \renewcommand{\arraystretch}{1.2}
  \centering
  \caption{Fair Coverage: Varying Number of IDFs}%
  \label{tab:centralized_vs_lpac_IDF_ablation}%
  \begin{tabular}{ccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\# IDFs}} &\multicolumn{2}{c}{\# Best Environments} & \multicolumn{2}{c}{Average Max Objective}\\\cmidrule(l){2-3} \cmidrule(l){4-5}
    \multicolumn{1}{c}{} & \multicolumn{1}{r}{Centralized CVT} & \multicolumn{1}{r}{LPAC} & \multicolumn{1}{r}{Centralized  CVT} & \multicolumn{1}{r}{LPAC}\\\midrule
4 & 6 & 94 & 2.251&1.386 \\
5 & 6 & 94 & 3.137&1.979 \\
6 & 5 & 95 & 4.144&2.486 \\
7 & 4 & 96 & 5.072&3.214 \\
8 & 4 & 96 & 6.144&3.792 \\
9 & 1 & 99 & 7.060&4.667 \\
10 & 0 & 100 & 8.104&5.037 \\
 \bottomrule
  \end{tabular}
\end{table}



\begin{figure*}
    \centering
    \subfloat[Robot ablation. The performance ratio between LPAC and Centralized as a function of time for the fair coverage control problem. We vary the number of robots by steps of $8$, from $8$ to $64$ with $1024\times 1024$ environment.]{%
        \includegraphics[width=0.3\textwidth]{plots/ratio_lpac_centralized_all_robots.pdf}
        \label{fig:fair_coverage_ablation}
    }
    \hfill
    \subfloat[Constraint Ablation. The performance ratio between LPAC and Centralized as a function of time for the fair coverage control problem. We vary the number of IDFs/constraints, from $4$ to $10$ IDFs with $1024\times 1024$ environment.]{%
        \includegraphics[width=0.3\textwidth]{plots/features_ratio_lpac_centralized_all_robots.pdf}
        \label{fig:features_fair_coverage_ablation}
    }
    \hfill
    \subfloat[Problem scale ablation. The performance ratio between LPAC and Centralized as a function of time in the fair coverage control problem. We vary the size of the environment and the number of robots, while maintaining the robot density.]{%
        \includegraphics[width=0.3\textwidth]{plots/env_size_ratio_lpac_centralized_all_robots.pdf}
        \label{fig:env_size_ratio_lpac_centralied_all_robots.pdf}
    }
    \caption{Comparison of LPAC and Centralized performance under different experimental setups in the fair coverage control problem: robot ablation, feature ablation, and problem scale ablation.}
    \label{fig:ablation_comparison}
\end{figure*}

\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{plots/constraint.pdf}
	\caption{Contraint coverage control with varying constraint levels. We plot the IDF infeasibility and problem infeasibility percentage. Accross all constraint levels, LPAC is infeasible in at least half of the IDFs, and Problems that are Centralized are infeasible.
 }
	\label{fig:constraint}
\end{figure}


% \red{add paragraph, explanation, from LPAC page 8. 3,4,5 horizontally alignment. }
% \red{Latex font - in plots.}
% \VK{Saurav, as I mentioned to you, the 1024 sq m, the sensing radius, and the comms radius need to be normalized. perhaps by the length of the square, 32m. Else it looks like a case study. Vijay}
% \sa{This is $1024\times1024$ environment. Juan, please make sure of this.}


% In this section, we showcase the benefits of our method on a multi-objective coverage control problem.
In this section, empirically study the two problems \textit{fair coverage} and \textit{constrained coverage}. 
The goal of the study is to show that : (i)~an efficient solves for the multi-objective coverage control problem, (ii) generalization to a wide range of robot parameters, (ii) generalization to unseen domains, (iii) scales with number of robots, number of IDFs, and environment size.


We compare our method against four baseline controllers: decentralized and centralized CVT, SFCC \cite{malenciafair}, and the clairvoyant algorithm. The centralized and decentralized CVTs are gradient descent algorithms that move the robots towards the center of inertia of each Voronoi partition based on decentralized or centralized information (see~\cite[Section V.A]{agarwal2024lpac}). These algorithms operate on the partial information about the IDF gathered by the robots throughout the trajectory and utilize the combination of IDFs. SFCC \cite{malenciafair} is a centralized gradient-based algorithm that operates on the $\textbf{LogSumExp}$ of the IDFs. The clairvoyant algorithm has perfect knowledge of all the IDFs and the positions of the robots and can, therefore, compute near-optimal actions for each robot. It is important to highlight that LPAC possesses the same local information as the decentralized CVT algorithm but that both centralized and clairvoyant have access to global data. 

\textbf{Fair Coverage.}
We begin by considering the fair coverage control problem defined in \eqref{eqn:epi_multi_objective_coverage}.
Figure~\ref{fig:fair_coverage} presents the maximum coverage cost across all IDFs averaged over $100$ randomly generated environments.
The LPAC outperforms centralized and decentralized CVT by $50\%$.
Moreover, considering the standard deviation bands around each mean, we see that the centralized and LPAC fall outside the mean curve.
The result illustrates the benefits of using GNNs for multi-objective coverage control, even when accessing partial decentralized information. 

Figure~\ref{fig:comm_radius} shows the performance of the LPAC algorithm with respect to the centralized solver as the communication radius and the sensor size of the robot are varied.
The centralized algorithm is agnostic to the communication radius and it's performance increases with sensor size; it is equivalent to the clairvoyant algorithm for very large sensor sizes.
The LPAC algorithm, on the other hand, is sensitive to the communication radius and the sensor size, and yet it consistently outperforms the centralized algorithm for all configurations.

In Figure \ref{fig:fair_objective_dual_variables} we plot the trajectories of the IDFs and the dual variables on the upper and lower rows respectively. 
% This environment helps us understand the role of the primal-dual algorithm in solving the multi-objective coverage problem. 
The upper row shows how the performance across IDFs improves as time progresses. 
% Interestingly, there are two distinct behaviors, the one by clairvoyant and LPAC on one side, and the centralized and decentralized CVT on the other side. 
The case of clairvoyant and LPAC present a switch on the most difficult IDF, from $1$ to $2$ around $15$ time steps. In the case of the CVT algorithm, it struggles throughout all the trajectories with IDF $1$. The value of the dual variable is proportional to the difficulty of satisfying the constraint, which, in this case, translates into minimizing that IDF. Therefore, the switch in the objective value also manifests as a switch in the maximum dual variable $\lambda$. 

In terms of scalability, we run an ablation study on the number of robots from $8$ robots to $64$ in steps of $8$. Figure \ref{fig:fair_coverage_ablation} shows the ablation study on the number of robots, in this case, we look at the ratio of the centralized controller by LPAC. We run $100$ experiments per number of robots and confirm that values are smaller than $1$ given that LPAC outperforms centralized CVT. We can see that when the number of robots is larger than $32$ (number of robots used for training), LPAC outperforms centralized CVT by more than $30\%$. Additionally, in Table \ref{tab:centralized_vs_lpac_fair_robot_ablation} we show the number of times that each controller attains the best performance. Here the LPAC becomes even more useful given that LPAC performs better than centralized CVT at least $94\%$ of the time. 

In Figure \ref{fig:features_fair_coverage_ablation} run an ablation study on the number of IDFs or constraints, starting at $4$ and ending at $10$. In this case, we show the scalability in terms of the number of constraints, and we confirm that LPAC outperforms centralized CVT by at least $35\%$ in all cases. Thus showcasing the ability of LPAC to operate under a larger number of constraints. 

In Figure \ref{fig:env_size_ratio_lpac_centralied_all_robots.pdf} we scale the problem in the size of the environment and robots jointly. Once again, LPAC outperforms the centralized CVT algorithm by at least $35\%$, thus showing that LPAC scales in the coverage control problem size. 
% \subsubsection{Scaling robots}
% Tests for 8 to 64 robots in steps of 8.
% The results are for centralized and LPAC over 500 steps, i.e., 20 dual updates.
% We can normalize LPAC wrt centralized and plot.

% % \url{https://drive.google.com/file/d/1Rx7u2Se9HRQw-GQBNG3-oiCaFPlyIdPy/view?usp=sharing}

% \subsubsection{Scaling features and number of idfs}
% Tests for 32 to 80 features in steps of 8, i.e., 32, 40, ..., 80.
% Number of idfs = number of features/8.
% The results are for centralized and LPAC over 500 steps, i.e., 20 dual updates.
% We can normalize LPAC wrt centralized and plot.

% \begin{figure*}[ht]
%   \centering
%   \includegraphics[width=\textwidth]{plots/env_72_plots_1_25.pdf}
%   \caption{Performance and dual variables per IDF as a function of time for $32$ robots and $4$ IDFs. }\label{fig:fair_objective_dual_variables}
% \end{figure*}
\textbf{Constraint Coverage Control.}
We consider the constrained coverage control problem \eqref{eqn:multi_objective_coverage}. In this case, we compared the centralized CVT against our formulation of LPAC. Note that to the best of our knowledge, there does not exist another algorithm to compare against for the multi-objective coverage control problem. We considered the feasibility problem, i.e. $\phi_0=0$, and sampled the constraints $\alpha_m$ according to $\ccalN(\mu,0.1)$, for $\mu\in\{0.3,\dots,0.9\}$, and considered $M=4$ IDFs.

In Figure \ref{fig:constraint} we plot the results, both in terms of the percentage of infeasible IDFs, as well as infeasible problems (at least one of the four IDFs is infeasible). As can be seen, the percentage of infeasible IDFs in LPAC is always less than half that in Centralized CVT. In terms of the problems, LPAC achieves an average of $25\%$ less infeasible problems across all $\mu$s. This showcases the benefits of our proposed approach for constrained multi-objective coverage control. 

